CertRL: Formalizing Convergence Proofs for Value and Policy Iteration in Coq

Reinforcement learning algorithms solve sequential decision-making problems in probabilistic environments by optimizing for long-term reward. The desire to use reinforcement learning in safety-critical settings inspires a recent line of work on formally constrained reinforcement learning; however, these methods place the implementation of the learning algorithm in their Trusted Computing Base. The crucial correctness property of these implementations is a guarantee that the learning algorithm converges to an optimal policy. This paper begins the work of closing this gap by developing a Coq formalization of two canonical reinforcement learning algorithms: value and policy iteration for finite state Markov decision processes. The central results are a formalization of Bellman's optimality principle and its proof, which uses a contraction property of Bellman optimality operator to establish that a sequence converges in the infinite horizon limit. The CertRL development exemplifies how the Giry monad and mechanized metric coinduction streamline optimality proofs for reinforcement learning algorithms. The CertRL library provides a general framework for proving properties about Markov decision processes and reinforcement learning algorithms, paving the way for further work on formalization of reinforcement learning algorithms.

==> extra.tex <==

The optimal value function of the Markov decision process of infinite length 
is defined as the limit
\begin{equation}
  \hat V_{*, \infty} := \lim_{t \to \infty} \hat V_{*, t}
\end{equation}

Again, like in the previous subsection, the limit of the iterative
sequence $\hat V_{*, t + 1} = \hat \bellman_{*} \hat V_{*, t}$ exists by Banach fixed
point theorem because the Bellman operator
$\hat \bellman_{*}: \reals^\states \to \reals^\states$ is a contraction mapping
in the max-norm ($L^\infty$-norm) on $\reals^\states$.

Now notice that for any length  $t \in \integers_{\geq 0}$ of a Markov decision process
and any policy sequence $\bar \pi = \pi_0::\pi_1::$
we have that 
\begin{equation}
  \hat V_{*, t} \geq V_{\bar \pi, t}
\end{equation}

In particular, for all $t \in \integers_{\geq 0}$, the above inequality holds
for stationary sequence of policies $\bar \pi = \pi::\pi::\dots::\pi$:
\begin{equation}
\forall \policy: \quad  \hat V_{*, t} \geq V_{\pi, t}
  \label{eq:inequality}
\end{equation}

Since weak inequality is preserved by limit, and the limits of $\hat V_{*, t}$ and $V_{\pi, t}$
exists (from Banach fixed point theorem applied to Banach optimality operator and Banach policy operator, respectively),
we conclude that
\begin{equation}
\forall \pi  \qquad  \hat V_{*, \infty} \geq V_{\pi, \infty}
\end{equation}

More explicitly, the recursion with Bellman operator $\bellman_{*}:$ can be presented
as
\begin{equation}
\forall s:   V_{*, t + 1}(s) = \sup_{a(s)} (Q_{*, t} (a, s))
\end{equation}
where \emph{action-value} function $Q_{*, t}: A \times S \to \mathbb {R}$  is defined as
\begin{equation}
  (Q_{*, t}) (a) := \bar v(a) + \gamma T(a) V_{*, t}
\end{equation}

The optimal policy for the first step of the Markov decision process of length (t + 1) is computed recursively
\begin{equation}
  a_{*, t + 1} (s) := \argmax_{a}  Q_{*, t} (a, s)
\label{eq:argmax}
\end{equation}
from the computed optimal value $V_{*, t}$ and optimal action-value
functions $Q_{*, t}$ for Markov decision processes of length t. The argmax is a multi-valued (set valued)
function, so that  $a_{*, t + 1}: \states \to \mathcal{P}(\actions)$ where $\mathcal{P}(\actions)$ denotes the powerset of $\actions$. 

The sequence for iterations $t = 0, 1, 2, \dots$ of set-valued functions $a_{*, t + 1}: \states \to \mathcal{P}(\actions)$ converges in the $t = \infty$ limit to (possibly multi-valued) optimal policy
\begin{equation}
  a_{*, \infty}(s) := \lim_{t \to \infty} a_{*, t}(s) = \argmax Q_{*, \infty} (a, s)
\end{equation}


==> related_2.tex <==
To our knowledge, \libname is the first formal proof of convergence for value iteration or policy iteration.
Related work falls into three categories: 
\begin{enumerate}
  \item libraries that our work builds upon,  
  \item formalizations of results from probability and machine learning, and
  \item work at the intersection of formal verification and reinforcement learning.
\end{enumerate}

\paragraph{Dependencies}
\libname builds on the Coquelicot \cite{Coquelicot} library for real analysis. 
Our main results are statements about fixed points of contractive maps in complete normed modules.
\libname therefore builds on the formal development of the Lax-Milgram theorem and, in particular, Boldo et al.'s formal proof of the Banach fixed point theorem \cite{BoldoElfic}.
\libname contains an implementation of the Giry monad. Our use of the monad for reasoning about probabilistic processes, as well as the design of our library, is highly motivated by the design of the Polaris library \cite{tassarotti2019separation}. Building on these other foundations, \libname demonstrates how existing work on formalization enables formalization of key results in reinforcement learning theory.

\paragraph{Related Formalizations}
There is a growing body of work on formalization of machine learning theory.
Of these,  Johannes H\"{o}lzl's Isabelle/HOL development of Markov Processes is most related to our own work \cite{markovInHOL}. 
H\"{o}lzl builds on the probability theory libraries of Isabelle/HOL to develop continuous-time Markov chains.
Many of H\"{o}lzl's basic design choices are similar to ours; for example, he also uses the Giry monad to place a monadic structure on probability spaces and also utilizes coinductive methods.
\libname focuses instead on formalization of convergence proofs for dynamic programming algorithms that solve Markov Decision Processes. In the future, we plan to extend our formalization to include convergence proofs for model-free methods, in which a fixed MDP is not known a priori.
\todo[inline]{
  We can cite \cite{tassarotti2019formal} but make explicit mention.
  If this is being cited because it's an ML formalization, maybe we do a cite checklist at the beginning.
  If this is being cited because it provides a survey, say something like ``Tass. et al. surveys teh state of this literatue... (cite that and any relevant papers).
}



The CertiGrad formalization by Selsam et al. contains a Lean proof that the gradients sampled by a stochastic computation graph are unbiased estimators of the true mathematical function \cite{DBLP:conf/icml/SelsamLD17}. 
This result, together with our development of a library for proving convergence of reinforcement learning algorithms, provides a path toward a formal proof of correctness for deep reinforcement learning.

\paragraph{Formal Methods for RL}
The likelihood that reinforcement learning algorithms will be deployed in safety-critical settings during the coming decades motivates a growing body of work on formal methods for safe reinforcement learning.
The basic approach -- variously called 
shielding \cite{DBLP:conf/aaai/AlshiekhBEKNT18}, 
formally constrained reinforcement learning \cite{HasanbeigKroening}, or
verifiably safe reinforcement learning \cite{aaai18} -- uses temporal or dynamic logics to specify constraints on the behavior of RL algorithms.

Global convergence is a fundamental theoretical property of classical reinforcement learning algorithms, and in practice at least local convergence is an important property for any useful reinforcement learning algorithm.
However, the formal proofs underlying these methods typically establish the correctness of a safety constraint but do not formalize any convergence properties for the underlying algorithms.
In future work, we plan to establish an end-to-end proof that constrained reinforcement learning safely converges by combining our current development with the VeriPhy pipeline of Bohrer et al. \cite{DBLP:conf/pldi/BohrerTMMP18}.

